Stein particle filtering

We present a new particle filtering algorithm for nonlinear systems in the discrete-time setting. Our algorithm is based on the Stein variational gradient descent (SVGD) framework, which is a general approach to sample from a target distribution. We merge the standard two-step paradigm in particle filtering into one step so that SVGD can be used. A distinguishing feature of the proposed algorithm is that, unlike most particle filtering methods, all the particles at any time step are equally weighted and thus no update on the weights is needed. We further extended our algorithm to allow for updating previous particles within a sliding window. This strategy may improve the reliability of the algorithm with respect to unexpected disturbance in the dynamics or outlier-measurements. The efficacy of the proposed algorithms is illustrated through several numerical examples in comparison with a standard particle filtering method.

==> Stein filtering/scripts/background.tex <==
\section{Background} \label{sec:backg}
% In this section we present the basic setup of particle filtering. We also provide a brief introduction to Stein variational gradient descent method, on which our particle filtering algorithms are based.

In this section,  we present the mathematical formulation of the nonlinear filtering problem in discrete-time setting, a brief description  the particle filter algorithm, and a brief introduction to the Stein variational gradient descent method.


\subsection{Nonlinear filtering problem}
Consider the following dynamical system 
\begin{subequations}\label{eq:dyn}
    \begin{eqnarray}\label{eq:dyn1}
        x_{t+1} &\sim& p(x_{t+1}\mid x_t),\quad x_1 \sim p(x_1),
        \\\label{eq:dyn2}
        z_t &\sim& p(z_t\mid x_t),
    \end{eqnarray}
\end{subequations}
for $t  \in \mathbb{N}$ where  $x_t \in \mR^d$  denotes the state of the system at time $t$, and $z_t \in \mR^l$ denotes the observation process. Here $p(x_{t+1}|x_t)$ represents the transition probability of the Markov process $x_t$ and $p(z_t|x_t)$ represents the likelihood function of observing $z_t$  given $x_t$. The objective of the filtering problem is to compute the posterior distribution $p(x_t|Z_t)$ where $Z_t:=\{z_1,\ldots,z_t\}$ denotes the history of observations up to time $t$.


The posterior distribution can be computed recursively in two steps, using the Markov property of $x_t$ and the Bayes rule. In particular, given $p(x_t|Z_t)$, the posterior distribution at the next time step $p(x_{t+1}|Z_{t+1})$ is given by:
\begin{subequations}\label{eq:one_step_dist}
\begin{align}
         p(x_{t+1}|Z_{t})
    %  & =\int_{x_t} p(x_{t+1},x_{t}|Z_t)          \\
    %  & =\int_{x_t} p(x_{t+1}|x_{t},Z_t)p(x_{t}|Z_t) \\
     & =\int_{x_t} p(x_{t+1}|x_{t})p(x_{t}|Z_t),\\
         p(x_{t+1}|Z_{t+1})
    %  & = \frac{p(z_{t+1}|x_{t+1},Z_t)p(x_{t+1}|Z_t)}{p(Z_{t+1})}  \\
    %  & = \frac{p(z_{t+1}|x_{t+1})p(x_{t+1},Z_t)}{p(Z_{t+1})}        \\
    %  & = \frac{p(z_{t+1}|x_{t+1})p(x_{t+1}|Z_t) p(Z_t)}{p(z_{t+1}|Z_t)p(Z_{t})} \\
     & =\frac{p(z_{t+1}|x_{t+1}) p(x_{t+1}|Z_t)}{p(z_{t+1}|Z_t)}.
\end{align}
\end{subequations}
Although the posterior admits a recursive update law in principle, it is numerically challenging to implement the update law in practice due to the fact  the posterior distribution is infinite-dimensional and    computation of the normalization constant is challenging. 


\subsection{SIR particle filter}
The main idea in particle filters is to approximate the posterior distribution with weighted empirical distribution of particles
\begin{equation}
    p(x_t|Z_t) \approx \sum_{i=1}^n w^i_t \delta_{x^i_t}
\end{equation}
such that $\sum_{i=1}^n w^i_t=1$, where $\delta_x$ is the Dirac delta distribution located at $x$. There are several standard variations of the particle filter that are being used in practice. Each variation corresponds to a different choice of proposal density to update the particle location and evaluate the importance sampling weights. In this paper, we consider the sequential importance resampling (SIR) particle filter where the particles are update according to the dynamic model leading to the following update law for particles and weights~\cite{arulampalam2002tutorial}   
\begin{align*}
    x^i_{t+1} &\sim p(x_{t+1}|x^i_t)\\
    w^i_{t+1} &= \frac{w^i_t p(z_{t+1}|x^i_{t+1})}{\sum_{j=1}^n w^j_t p(z_{t+1}|x^j_{t+1})}. 
\end{align*}
To avoid the weight degeneracy issue, a resampling step is carried out after several steps, where $n$ independent new samples are generated from the weighted distribution $\tilde{x}^i_t \sim \sum_{i=1}^n w^i_t \delta_{x^i_t}$. After the resampling procedure, the posterior distribution is approximated with empirical distribution of the new samples with equal weights, i.e. $p(x_t|Z_t) \approx \frac{1}{n}\sum_{i=1}^n \delta_{\tilde{x}^i_t}$.  

% \subsection{Particle filtering}
% \jiaojiao{The particle filtering paradigm utilizes the particle representation of the posterior distribution and iteratively updates the particles as new measurements become available.}
% % The iteration is based on the Bayesian formula in Equation (\ref{eq:one_step_dist}).

% Given a dynamical system
% \begin{subequations}\label{eq:dyn}
%     \begin{eqnarray}\label{eq:dyn1}
%         x_{t+1} &\sim& p(x_{t+1}\mid x_t),\quad x_1 \sim p(x_1)
%         \\\label{eq:dyn2}
%         z_t &\sim& p(z_t\mid x_t),
%     \end{eqnarray}
% \end{subequations}
% % where $f: \mR^d \times \mR^d \rightarrow \mR^d$ and $g: \mR^l \times \mR^l \rightarrow \mR^l$ are the given function, 
% with state $x_t \in \mR^d $ and measurement $z_t \in \mR^l$,
% % $x_0, x_1, \cdots$ is a Markov process, where the probability of $x_t$ only depends on $x_{t-1}$. Likewise, $p(z_t)$ only depends $x_t$. The Markov process is revealed in Figure \ref{fig:pf}.
% denoting by $Z_t:=\{z_1, z_2, \ldots, z_t\}$ all the past measurements,
% the filtering problem aims at computing/estimating posterior distribution $p(x_t | Z_t)$ for $t=1,2,3, \cdots$.
% % \begin{figure}[ht]
% %     \begin{center}
% %         \centerline{\includegraphics[width=0.98\columnwidth]{plot/pf.pdf}  }
% %         \caption{
% %             particle filtering}
% %         \label{fig:pf}
% %     \end{center}
% %     \vskip -0.2in
% % \end{figure}

% Thanks to the Bayes Rule and the Markov property of the process,
% % the particle filtering problem could be transformed to solving the posterior distribution of $x_t$ at time $t$. At time $t+1$, given the observations $Z_{t+1}$, 
% the posterior distribution $p(x_{t+1}|Z_{t+1})$ at time $t+1$ reads
% \begin{align*}
%     p(x_{t+1}|Z_{t+1})
%      & = \frac{p(z_{t+1}|x_{t+1},Z_t)p(x_{t+1},Z_t)}{p(Z_{t+1})}  \\
%     %  & = \frac{p(z_{t+1}|x_{t+1})p(x_{t+1},Z_t)}{p(Z_{t+1})}        \\
%     %  & = \frac{p(z_{t+1}|x_{t+1})p(x_{t+1}|Z_t) p(Z_t)}{p(z_{t+1}|Z_t)p(Z_{t})} \\
%      & =\frac{p(z_{t+1}|x_{t+1}) p(x_{t+1}|Z_t)}{p(z_{t+1}|Z_t)}.
% \end{align*}
% % where in the second equation we use the Markov process assumption. $p(z_{t+1}|x_{t+1})$ is given by the function $h$ and noise $w_t$, 
% Note that $p(z_{t+1}|Z_{t})$ is determined by the measurement and can be treated as a constant in the filtering problem.
% The predicted distribution $p(x_{t+1}|Z_t)$ relates to the posterior distribution $p(x_{t}|Z_t)$ at the previous step through
% % is With the help of Bayes rule, we can break down $p(x_{t+1}|Z_t)$ ahead,
% \begin{align*}
%     p(x_{t+1}|Z_{t})
%      & =\int_{x_t} p(x_{t+1},x_{t}|Z_t)          \\
%     %  & =\int_{x_t} p(x_{t+1}|x_{t},Z_t)p(x_{t}|Z_t) \\
%      & =\int_{x_t} p(x_{t+1}|x_{t})p(x_{t}|Z_t).
% \end{align*}
% % $p(x_{t}|Z_t)$ is the result of last timestamp particle filtering. 
% % Thus we can establish connection between different timestamp posterior distribution as follows
% The above argument leads to an iterative update of the posterior distribution as follows
% \begin{equation}
%     p(x_{t+1} | Z_{t+1}) = \frac{\int_{x_t} p(x_{t+1}|x_t) p(x_t | Z_t) p(z_{t+1} | x_{t+1})}{p(z_{t+1} | Z_t)}.
%     \label{eq:one_step_dist}
% \end{equation}
% % In this article we target to tackle with discrete dynamics systems. We adopt Kalman filter and sampling importance resampling (SIR) filter as the benchmark.

% % \paragraph{Kalman filter}
% % Kalman filter gives the optimal solution for Linear system with Gaussian noise. It interchangeably does prediction and update with closed form solution.

% % \paragraph{Sampling Importance Resampling filter}
% % SIR algorithm is a Monte Carlo method that could deal with nonlinear dynamics with non-Gaussian noise. 

% The particle filtering framework is an realization of the above iterative update \eqref{eq:one_step_dist} using particle representation.
% \jiaojiao{In particular, $p(x_{t+1}|x_t)$ and $p(z_{t+1} | x_{t+1})$ are determined by $f$ and $g$ respectively. And the posterior distribution $p(x_{t}|Z_t)$ is captured by $N$ particles $\{x_t^i\}_{i=1}^N$ and the associated weights $\{w_t^i\}_{i=1}^N$ ($\sum w_t^i=1$).} 

% \jiaojiao{In the sequential important resampling (SIR) particle filter,
%     % {\red improve the following}
% % Without accessed closed-form solution, it depicts distributions with particles $\{x_t^i\}_{i=1}^N$ instead.
% % Each particle carries a weight $a_t^i$ which characterize the "importance" of this particle for representing the distribution. 
% at time $t+1$, one always samples $x_{t+1}^i \sim p(x_{t+1}|x_{t}^i)$ and then adjusts the accompanying weights $w_{t+1}^i=w_{t}^i \cdot p(z_{t+1}|x_{t+1}^i)$ accordingly \cite{arulampalam2002tutorial}.
% % an often used prior distribution to sample particles is $\widehat{x}_{t+1}^i \sim p(x_{t+1}|x_{t}^i)$. Then it could be proved that $w_{t+1}^i=w_{t}^i \cdot p(z_{t+1}|x_{t+1}^i)$ \cite{arulampalam2002tutorial}. 
% To avoid the weight degeneracy phenomenon, which is that the effective sampling size is low, a resampling process will be adopted after the weight update. Resampling would generate a set of new particles that are associated with roughly equal weights.}


% {\red
%     % 1. problem formulation of filtering\\
%     % 2. Sequential Bayesian update\\
%     % 3. SIR implementation
% }


==> Stein filtering/scripts/introduction.tex <==

\section{Introduction}
% \jiaojiao{1. What's particle filtering?\\
% 	2. Why is it important? applications?\\
% 	3. Computational challenge, what has been done?\\
% 	4. our goal, Our proposed method?\\
% 	5. Summary of contribution. Why is our method good?\\
% 	6. Related work\\
% }

% {\red
%     1. Filtering is important and has many applications.\\
%     2. Particle filtering is a filtering algorithm. What's particle filtering? Advantages? Limitations?\\
%     3. Our goal\\
%     4. Our proposed method\\
%     5. advantages of our method\\
%     6. related work
% }


Particle filters are sequential Monte-Carlo based algorithms designed to numerically approximate the solution to the filtering problem~\cite{gordon1993novel,doucet2009tutorial}. The basic idea in particle filter is to approximate the posterior distribution with weighted empirical distribution of particles. The key step in approximation is importance sampling, where the weights of the particles are updated according to the Bayes rule that involves the likelihood of the observation signal. The issue with this approach is that after several time-steps, there are only a few particles with large wights, while most of the particles have nearly zero weights. This issue is referred to as particle degeneracy~\cite{gordon2004beyond}. To mitigate the issue, particle filters perform a resampling step, where new independent particles with uniform weights are sampled from the weighted empirical distribution. Theoretically, it is shown that the particle filters are exact as the number of particles grows to infinity, with error rate $O(N^{-\frac{1}{2}})$~\cite{del2001stability,cappe2006inference}. However, both empirically and theoretically, it was discovered that particle filters perform poorly in high-dimensional problems~\cite{bengtsson2008curse,beskos2014error,rebeschini2015can}.
% to maintain the same amount of error, the number of particles should grow exponentially with dimension, a phenomenon known as curse of dimensionality

In this work, we propose a particle filtering framework which doesn't suffer from particle degeneracy. Departing from most particle filtering methods which iteratively update the weights of the particles through important sampling, our approach iteratively update only the locations of the particles. Consequently, all the particles at each time step remain uniformly weighted throughout. Thus, the effective particle size remains high all the time, a desirable property for particle filtering, particularly for high-dimensional applications. 

Our particle filtering method is based on the Stein variational gradient descent (SVGD) framework. The latter is a general purpose sampling technique which can generate samples from any given probability density as Markov chain Monte Carlo (MCMC) methods. One major difference between SVGD and MCMC is that the samples generated using SVGD are deterministic. It was argued that SVGD is less vulnerable to mode collapse than MCMC \cite{LiuWan16}. Moreover, the SVGD only need to know the target probability density up to a normalization factor. Thus, it is suitable for sampling from posterior distribution where the normalization factor is not available. In our method, we approximate the posterior distribution up to a normalization factor of the next time step using the particles of the current step and the next measurement. With this approximated posterior distribution we can adopt SVGD to sample from it. Our particle filtering algorithm is an iterative implementation of SVGD in this manner.
% makes use of particles to perform gradient descent over the functional space to gradually approach a target distribution with a given initialized distribution.

A sliding window version of this algorithm is also developed. It iteratively samples the trajectories of the posterior dynamics over a fixed-size sliding window instead of one-time point. In this sliding window particle filtering algorithm, each measurement is used multiple times as each measurement belongs to several different sliding windows. This reuse of measurement is helpful to improve the tolerance of the algorithm to mistakes made at some time step. Another potential benefit of this method is higher robustness with respect to outlier observations. 
% On the other hand, to estimate the internal states $x_t $, we hope to reuse the observations $z_t$ for multiple times to calculate the posterior distribution. Thus we propose the sliding window Stein particle filtering. The idea of this method is instead of estimating the posterior distribution $p(x_t|z_{1:t})$, we switch to a joint conditional distribution $p(x_{t+1:t+T}|z_{1:t+T})$. 
% The advantage of this is one can leverage a longer record of observations to derive the Bayesian inference distribution. So the utilization rate of the observation at each time could rise up. This may mitigate the estimation error that is accumulated during the filtering.

% {\chen 
% Related works:
One standard particle filter is Sampling Importance Resampling particle filter (SIR), which has been shown to be stable and well-performed in various settings. 
% There are some other variants such as auxiliary sampling importance resampling (ASIR) filter and regularized particle filter (RPF) \cite{doucet2009tutorial}. Feedback particle filter is an counterpart to SIR particle filter replacing the importance sampling step with the feedback control \cite{yang2013feedback,taghvaei2020diffusion}. 
% }
% \amir{
There is a growing interest in developing nonlinear   filter algorithms that avoid the weight degeneracy issue in particle filters by replacing the importance sampling step with a control-based approach. There are identified under the category of controlled interacting particle systems. The earliest example is the ensemble Kalman filters~\cite{evensen1994sequential,bergemann2012ensemble} which provides an exact solution to the filtering problem in linear Gaussian setting and has been widely applied in meteorological applications.  Feedback particle filter~\cite{yang2013feedback,yang2016multivariable,taghvaei2020diffusion} provides generalization of the ensemble Kalman filter to nonlinear and non-Gaussian setting~\cite{taghvaei2018kalman}. Other examples of controlled interacting particle systems include Crisan and Xiong filter~\cite{crisan2005approximate}, particle flow filters~\cite{daum2010exact}, and ensemble transform particle filter~\cite{reich2013nonparametric}. 
% }

The rest of the paper develops as follows. In Section \ref{sec:backg} we present the background on particle filtering and the Stein variational gradient descent method. The proposed particle filtering algorithms are presented in Section \ref{sec:stein}. It is followed by several numerical examples in Section \ref{sec:num} and a concluding remark in Section \ref{sec:conclusion}.

% We firstly would like to bring forward a method that doesn't require importance sampling framework. Stein variational gradient descent (SVGD) makes use of particles to perform gradient descent over the functional space to gradually approach a target distribution with a given initialized distribution.

% On the other hand, to estimate the internal states $x_t $, we hope to reuse the observations $z_t$ for multiple times to calculate the posterior distribution. Thus we propose the sliding window Stein particle filtering. The idea of this method is instead of estimating the posterior distribution $p(x_t|z_{1:t})$, we switch to a joint conditional distribution $p(x_{t+1:t+T}|z_{1:t+T})$. The advantage of this is one can leverage a longer record of observations to derive the Bayesian inference distribution. So the utilization rate of the observation at each time could rise up. This may mitigate the estimation error that is accumulated during the filtering.

% Earliest particle filters include Sampling Importance Resampling particle filter (SIR), which has shown to be stable and well-performed in many situations. There are some other variants like auxiliary sampling importance resampling (ASIR) filter and regularized particle filter (RPF) \cite{doucet2009tutorial}. Feedback particle filter is an counterpart to SIR particle filter replacing the importance sampling with the feedback control.

% The contribution of our paper has two folds: 1) we propose a novel Stein particle filtering framework, which provides a new insight to do particle filtering from gradient flow perspective; 2) we introduce a sliding window version particle filter, which could make use of a single observation for multiple times and decrease the estimation error.

% The paper develops as follows. In Section \ref{sec:backg} we present the background for particle filter and Stein variational gradient descent. In Section \ref{sec:stein} we introduce two methods leveraging SVGD to solve particle filtering. In Section \ref{sec:num} we give numerical example to verify our algorithms.

==> Stein filtering/scripts/numerical.tex <==

\section{Numerical examples} \label{sec:num}
% In this section we provide both linear and nonlinear examples to verify our algorithm performance. We compare with SIR to evaluate the efficacy. In both the examples, we set the number of iteration $L=100$ and step size $\epsilon_l=0.01$ in our Stein method. We consider using 500 particles for each method.
% In Stein methods, we use step size $\epsilon_\ell=0.01$ and number of iteration $L=100$ for all the examples.
{
In this section, we provide numerical examples to evaluate the performance of our proposed algorithm in comparison with the SIR particle filtering algorithm. In all the reported numerical experiments, the number of particles of our algorithm and SIR particle filter are the same, equal to $n = 500$.  For the SVGD Algorithm~\ref{al:svgd}, the iteration number $L=100$, and the step-size $\epsilon_\ell = 0.01$. 
}
%  For linear example, we compare with Kalman Filter and SIR. For nonlinear example, we only compare with SIR.

\subsection{Linear Gaussian Setting}
% We consider the same linear system as the Section V.A in \cite{yang2013feedback}:
Consider the following continuous-time filtering problem with linear dynamics, linear observation model, and Gaussian prior distribution:
\begin{subequations}
    \begin{eqnarray}
        dx_t &=& -\frac{1}{2} x_t dt+dW_t,\quad x_0 \sim \cN(1,1) \\
        dy_t &=& 3 x_t dt+ \frac{1}{2} dV_t, 
    \end{eqnarray}
\end{subequations}
where $\{W_t\}$, $\{V_t\}$ are mutually independent standard Wiener processes. The solution to this filtering problem is explicitly known, given by the Kalman-Bucy filter~\cite{kalman1961new}. The posterior distribution is Gaussian $\cN(\mu_t,\Sigma_t)$ with the update law for mean and covariance as follows:
\begin{subequations}
    \begin{align}
        d \mu_t &= -\frac{1}{2} \mu_t dt + K_t(d y_t - 3 \mu_t dt)\\
        \frac{d \Sigma_t}{d t}  &= - \Sigma_t + 1 - 36\Sigma_t^2
    \end{align}
\end{subequations}
where $K_t = 12\Sigma_t$ is the Kalman gain. 

% This is equivalent to $dW_t, dV_t \sim \cN(0, dt)$. We choose parameters as: $dt=0.02, \alpha=-0.5, \gamma=3, \sigma_W=0.5$. The total simulated time length is 10 seconds, which contains 1000 time steps.
% \begin{subequations}
%     \begin{eqnarray}
%         \bx_{t+1} &=& [[1,dt],[0,1]] \bx_t + Q \cdot N(0,[[9dt,0],[0,dt]])\\
%         \bz_t &=& [1,0] \bx_t +   \cN(0,R) ,\text{ try divide it by dt!!!}
%     \end{eqnarray}
% \end{subequations}
% As such discretization and denote $z_t={dy_t}/{dt}$, the simulated dynamics becomes
% \begin{subequations}
%     \begin{eqnarray}
%         x_{t+1} &=& (1+ \alpha dt) x_t + w_t, \quad w_t \sim \cN(0,dt),\\
%         z_t &=& \gamma x_t +v_t \quad v_t \sim  N\left(0,\frac{\sigma_W^2}{dt}\right).
%     \end{eqnarray}
% \end{subequations}
In order to implement our proposed algorithm and the SIR particle filter, the  continuous-time system is discretized according to
\begin{subequations}
    \begin{align}
       x_{t+\Delta t} &= (1-\frac{1}{2}\Delta t )  x_t + W_{t+\Delta t} - W_t,\\
         z_t := \frac{y_{t+\Delta t} - y_{t}}{\Delta t}  &= 3 x_t  +\frac{1}{2\Delta t}(V_{t+\Delta t} - V_t) 
        %  \quad v_t \sim  N\left(0,\frac{\sigma_W^2}{dt}\right).
    \end{align}
\end{subequations}
% \begin{subequations}
% \begin{align}
%  x_{t+\Delta t} - x_t &= –0.5\Delta t  x_t +  W_{t+\Delta t} - W_t , \quad x_0 \sim N(1,1)\\
%  y_{t+\Delta t} - y{t}  & = 3x_t \Delta t + 0.5 ( V_{t+\Delta t} - V_t) ,
% \end{align}
% \end{subequations}
where time step-size $\Delta t = 0.02$, and we introduced the discrete-time observation signal $z_t$. The increment of the Wiener process $W_{t+\Delta t} - W_t$ and $V_{t+\Delta t} - V_t$  is simulated by sampling independent  Gaussian random variables from $\cN(0,{\Delta t})$.

% To evaluate the performance of SIR and Stein methods, we compute the mean squared error of conditional mean and covariance after $M=50$ runs:
In order to measure the performance of the filtering algorithm, we use the mean-square-error criteria for estimating the conditional and the conditional covariance, averaged over $M=50$ independent runs: 
\begin{subequations}
\begin{align}
    \text{ m.s.e}_t^\mu   & =\frac{1}{M} \sum_{m=1}^M \left( \mu^{(n)}_t  - \mu_t \right)^2 , \label{mean mse}      \\
    % \mu^{(n)}_t       & =\frac{1}{n} \sum_{i=1}^n x^i_t,  \nonumber                                                     \\
    \text{m.s.e.}_t^\Sigma & =\frac{1}{M} \sum_{m=1}^M \left(  \Sigma^{(n)}_t - \Sigma_t \right)^2, \label{cov mse}          
%   \Sigma^{(N)}_t    & =\frac{1}{n-1} \sum_{i=1}^n (x_t^i-\mu^{(N)}_t)^2,\nonumber
\end{align}
\end{subequations}
where $\mu^{(n)}_t$ and $\Sigma^{(n)}_t$ are empirical mean and covariance of the particles given by
\begin{subequations}
\begin{align}
    % \text{ m.s.e}_t^\mu   & =\frac{1}{M} \sum_{m=1}^M \left( \mu^{(n)}_t  - \mu_t \right)^2 , \label{mean mse}      \\
    \mu^{(n)}_t       & =\frac{1}{n} \sum_{i=1}^n x^i_t,        \quad 
           \Sigma^{(n)}_t    & =\frac{1}{n-1} \sum_{i=1}^n (x_t^i-\mu^{(n)}_t)^2,\nonumber
\end{align}
\end{subequations}

The numerical result of the m.s.e. error for our proposed algorithm with stride $T=1$ and $T=3$, and the SIR particle filter are depicted in Figure~\ref{fig:linear}. It is observed that our proposed algorithm  admits smaller error compared to SIR with either choice of window length $T=1,3$. Among the two choices for time window, the one with $T=1$ admits slightly smaller error which is probably due to the fact that the particles in this case belong to $\mathbb{R}$, while in $T=3$, the particles belong to $\mathbb{R}^3$. We conjecture the optimization in a higher dimensional space could jeopardize the performance.


% In the following discussion, the stride $T=1$ means the Iterative Stein particle filtering method and the stride $T>1$ means the Sliding window Stein particle filtering method with window length $T$.
% We consider the case where the ratio between covariance and $x$ and $R$ is roughly 1. We observe that when ratio is around 1~5, the stride=1 could outperform stride=2,3,4... 
\begin{figure}[h]
    \centering
    \begin{subfloat}[m.s.e. for mean \label{fig:linear_mean}]
        { \includegraphics[width=0.95\linewidth]{images/mse_mean_linear.png}}
    \end{subfloat}

    \begin{subfloat}[m.s.e. for covariance \label{fig:linear_cov}]
        {\includegraphics[width=0.95\linewidth]{images/mse_cov_linear.png}}
    \end{subfloat}
    \caption{Numerical comparison of the filtering algorithms: Stein method and SIR particle filter, for the Linear Gaussian example}
    \label{fig:linear}
\end{figure}
% \begin{figure}[h]
%     \centering
%     \begin{subfloat}[mean]
%         { \includegraphics[width=0.48\linewidth]{images/mse_mean_linear_stride1.png}}
%     \end{subfloat}
%     \hfill
%     \begin{subfloat}[cov]
%         {\includegraphics[width=0.48\linewidth]{images/mse_cov_linear_stride1.png}}
%     \end{subfloat}
%     \caption{Linear example with Stein method stride $T=1$}
%     \label{fig:linear1}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfloat}[mean]
%         { \includegraphics[width=0.48\linewidth]{images/mse_mean_linear_stride3.png}}
%     \end{subfloat}
%     \hfill
%     \begin{subfloat}[cov]
%         {\includegraphics[width=0.48\linewidth]{images/mse_cov_linear_stride3.png}}
%     \end{subfloat}
%     \caption{Linear example with Stein method stride $T=3$}
%     \label{fig:linear3}
% \end{figure}

% From Figure \ref{fig:linear}, it could be told that the error goes larger when we increase the stride from 1 to 3. We conjecture this is because when the stride goes higher, SVGD is over a higher dimension (from $\mR^d$ to $\mR^{Td}$) and may jeopardize the performance.

\subsection{Nonlinear Case}
Consider the Benes filtering problem
\begin{subequations}
    \begin{eqnarray}
        dx_{t} &=& \mu \sigma_B \tanh\left(\frac{\mu}{\sigma_B }x_t \right) dt+\sigma_B dW_t, \\
        dy_t &=& (h_1x_t +h_1h_2)dt +dV_t,
    \end{eqnarray}
\end{subequations}
with $\mu=0.1$, $\sigma_B=0.3$, $h_1=5$, and $h_2=0$.  

% The total simulated time length is 10 seconds. After discretization, we have
% \begin{subequations}
%     \begin{eqnarray}
%         x_{t+1} &=& x_t+ \mu \sigma_B \tanh\left(\frac{\mu}{\sigma_B }x_t \right) dt +w_t, \\
%         z_t &=& h_1x_t +h_1h_2 +v_t, \\
%         w_t &\sim & \cN(0, \sigma_B^2), \\
%         v_t &\sim & N\left(0, \frac{1}{dt} \right).
%     \end{eqnarray}
% \end{subequations}
The closed-form solution of Benes filter is a mixture of two Gaussians~\cite[Ch. 6]{bain2008fundamentals}:
\begin{align*}
    c_t \cN(a_t-b_t,\sigma_t^2)+(1-c_t)\cN(a_t+b_t,\sigma_t^2),
\end{align*}
where
\begin{align*}
    a_t        & =  \sigma_B \Psi_t \tanh(h_1 \sigma_B t)+\frac{h_2+x_0}{\cosh(h_1 \sigma_B t)} -h_2, \\
    b_t        & =  \frac{\mu}{h_1} \tanh(h_1 \sigma_B t),                                            \\
    \sigma_t^2 & =  \frac{\sigma_B}{h_1} \tanh(h_1 \sigma_B t) ,                                      \\
    \Psi_t^2   & = \int_0^t \frac{\sinh(h_1 \sigma_B s)}{\sinh(h_1 \sigma_B t)} dY_s ,                \\
    c_t        & =  \frac{1}{1+e^{\frac{2a_tb_t}{\sigma_B} \coth(h_1 \sigma_B t)}}.
\end{align*}

\begin{figure}[h]
    \centering
    \begin{subfloat}[posterior density \label{fig:benes_density}]
        {\includegraphics[width=0.95\linewidth]{images/kde.png}}
    \end{subfloat}
    
    \begin{subfloat}[m.s.e. of the mean \label{fig:benes_mean}]
        { \includegraphics[width=0.95\linewidth]{images/mse_mean_nonlinear.png}}
    \end{subfloat}
    \caption{Numerical comparison of the filtering algorithms, Stein method and SIR particle filter, for the Benes filter. }
    \label{fig:benes}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfloat}[posterior density]
%         {\includegraphics[width=0.48\linewidth]{images/kde_stride2.png}}
%     \end{subfloat}
%     \hfill
%     \begin{subfloat}[mean]
%         { \includegraphics[width=0.48\linewidth]{images/mse_mean_benes_stride2.png}}
%     \end{subfloat}
%     \caption{Nonlinear example with Stein method stride $T=2$}
%     \label{fig:benes3}
% \end{figure}
In order to implement our algorithm and the SIR particle filter, we discretize the continuous-time model similar to the linear Gaussian case  with time step-size $\Delta t = 0.02$.  The numerical results for the Benes filter is depicted in Figure~\ref{fig:benes}. The sub-figure~\ref{fig:benes_density} depicts the exact posterior distribution along with the distributions of particles from the filtering algorithms at three time instants. In order to evaluate the density from particles, we used a kernel density estimation (KDE) with Gaussian kernel with bandwidth $0.1$.  The sub-figure~\ref{fig:benes_mean} depicts the m.s.e. error of the mean defined according to Equation~\eqref{mean mse} averaged over $M=50$ independent runs. It is observed that the Stein method with time window $T=3$ admits smaller error. This example demonstrates the advantage of using a time-window. It seems that in this case, the advantage of processing more observation signal  surpasses the error brought by simulating over a higher dimensional space.  
% This shows in this case, the advantage of using more observations surpasses the error brought by optimization over a higher dimension space. 
% It proves that increasing Stein particle filtering stride is a trade-off leveraging using more observations to decrease estimation error as well as the weak point that it would optimize over a higher dimension.


% We calculate the exact filtering solution and then get the mean squared error by taking 50 times run. From Figure \ref{fig:benes_mean}, it could be told that the error goes smaller when we increase the stride from 1 to 2. 
% This shows in this case, the advantage of using more observations surpasses the error brought by optimization over a higher dimension space. It proves that increasing Stein particle filtering stride is a trade-off leveraging using more observations to decrease estimation error as well as the weak point that it would optimize over a higher dimension.

==> Stein filtering/scripts/stein.tex <==

\section{Stein particle filtering} \label{sec:stein}

In this section, we propose stein particle filtering algorithm to iteratively estimate the posterior distribution $p(x_t|Z_t)$. It replaces the important sampling step in traditional particle filtering such as SIR with SVGD. As a result, the proposed algorithm only updates the position of the particles as the weights remain uniform throughout.
We present two variations of the algorithm: Sequential Stein particle filtering and Sliding window Stein particle filtering. The former sequentially update the particles to approximate $p(x_{t+1}|Z_{t+1})$ based on the particles that approximate $p(x_t|Z_t)$ as in most particle filtering algorithms. It only updates the particles associated with posterior distribution at the current step. The latter updates the particles for previous steps as well up to a fixed-size time window.
% They exhibit advantage in different application scenarios.

% We have some assumptions for Stein method to work on particle filtering setting. 1) The noise $w_t$ and $v_t$ distributions are given and we have the ability to sample from them. 2) The particle filtering problem starts with $t=1$ and the initial state distribution $p(x_1)$ is known.

\subsection{Sequential Stein particle filtering}
% Suppose
% $t \geq 1$ and  
In the Sequential Stein particle filtering algorithm, the posterior distribution 
$p(x_t |Z_t)$ is approximated by empirical distribution of $n$ particles $\{x_t^i\}_{i=1}^n$ with equal weights according to $p(x_t|Z_t) \approx \frac{1}{n} \sum_{i=1}^n \delta_{x^i_t}$. For $t>1$,  upon using this approximation in Equation \eqref{eq:one_step_dist}, we have the  the following expression for the posterior at the next time step:
\begin{equation}
    \label{eq:stride1_numeric}
    p(x_{t+1} | Z_{t+1}) \propto \left[\frac{1}{n} \sum_{i=1}^n p(x_{t+1}|x_t^i)\right] p(z_{t+1}|x_{t+1}).
\end{equation}
The main idea of the proposed algorithm is to apply the SVGD algorithm (Algorithm \ref{al:svgd}) to sample $n$ particles $x^i_{t+1}$ from the posterior $p(x_{t+1} | Z_{t+1})$. Then, this new set of particles are used to approximate the posterior distribution $p(x_{t+1} | Z_{t+1})$. This approximation is then used for the sampling of the next step. For $t=1$, the particles $x^i_1$ are generated by implementing the SVGD algorithm to sample from $p(x_{1}|Z_{1})$ given by 
\begin{equation}\label{eq:one_step_p1}
    p(x_{1} | Z_{1}) \propto p(z_1|x_1)p(x_1).
\end{equation}

There are two approaches to initialize the particles for implementing the SVGD algorithm in the particle filtering problems:  the particles can be initialized from  $x^i_t$, or they can be sampled from the Markov transition probability  $p(x^i_{t+1}|x^i_t)$. Numerically, we observed that the  latter initialization is more effective as it gives samples that are closer to the desired posterior distribution.
We name this algorithm the Stein particle filtering algorithm and present the details in {Algorithm \ref{al:Iterative}}. 

% However, when $t=0$, the case is more special. Given $p(x_1)$, we can get $p(x_{t+1}|Z_{t+1})$ as below
% \begin{equation*}\label{eq:one_step_p1}
%     p(x_{1} | Z_{
%             1}) \propto p(z_1|x_1)p(x_1).
% \end{equation*}
% % And by sampling $n$ particles $\tilde{x}_1^i \sim p(x_1)$, we can approximate
% % \begin{equation}
% %     \label{eq:one_step_p1}
% %     p(x_{1} | Z_{
% %             1}) \propto \left[ \frac{1}{n} \sum_{i=1}^n \tilde{x}_1^i \right] p(z_1|x_1).
% % \end{equation}
%  SVGD can be used to sample from $p(x_1|Z_1)$ straightforward.

% Note that this Stein particle filtering algorithm highly relies on the precision of $\{x^i_t\}_{i=1}^n$ because there is no "correction" step like Kalman filter. If $\{x^i_t\}_{i=1}^n$ fails to represent $p(x_t|Z_t)$ precisely, the Equation (\ref{eq:stride1_numeric}) would introduce error and this error would accumulate as time goes by. This would cause the estimated state distribution variance diverges. \amir{the error does not accumulate if the filter equation is stable}

\begin{algorithm}[tb]
    \caption{Sequential Stein particle filtering}
    \label{al:Iterative}
    \begin{algorithmic}
        \IF{$t=0$}
        \STATE {\bfseries Input:} initial dist. $p(x_1)$, observation $Z_1$
        % , step size $\epsilon_\ell$,
        % \STATE { \bfseries Initialize $x_{1,0}^i \sim p(x_1), i=1,2, \ldots, n$}
        \STATE {\bfseries Initialize:} $x^i \sim p(x_1), i=1,2, \ldots, n$
        \STATE {\bfseries Compute:} $\{\hat{x}^i\}=\text{SVGD}\left(p(x_{1}|Z_{1}),\{x^i \} \right) $ with Algorithm \ref{al:svgd}.
        % \FOR{$\ell=0,\ldots,L-1$}
        % \STATE { $ x_{1,\ell+1}^i=x_{1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{1,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{1}|Z_{1})$ in Equation (\ref{eq:one_step_p1}).
        % }
        % \ENDFOR
        \STATE {\bfseries Output: $\{x_{1}^i\}_{i=1}^n=\{\hat{x}^i\}_{i=1}^n$}
        \ELSIF{$t \geq 1$}
        \STATE {\bfseries Input:}
        $n$ particles from the last time step $\{x_{t}^i\}_{i=1}^n \sim p(x_t|Z_t)$, observations $Z_t$
        % , step size $\epsilon_\ell$
        \STATE { \bfseries Initialize $x^i \sim p(x_{t+1}|x_t^i), i=1,2, \ldots, n$}
        \STATE {\bfseries Compute:} $\{\hat{x}^i\}=\text{SVGD}\left(p(x_{t+1}|Z_{t+1}),\{x^i \} \right) $.
        % \FOR{$\ell=0,\ldots,L-1$}
        % \STATE { $ x_{t+1,\ell+1}^i=x_{t+1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{t+1,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{t+1}|Z_{t+1})$ in Equation (\ref{eq:stride1_numeric}).
        % }
        % \ENDFOR
        \STATE {\bfseries Output:  $\{x_{t+1}^i\}_{i=1}^n=\{\hat{x}^i\}_{i=1}^n$}
        \ENDIF
    \end{algorithmic}
\end{algorithm}

\subsection{Sliding window Stein particle filtering}
We next present a sliding window version of the Stein particle filtering algorithm. The main idea is to approximate the posterior distribution $p(x_{t+1:t+T} | Z_{t+T})$ over state trajectories of length $T$ recursively. When $t=0$, we sample from $p(x_1|Z_1)$ the same as Equation (\ref{eq:one_step_p1}).
When $1 \leq t < T$, the number of observations are not enough to form a window. By the Bayesian formula,
\begin{align}
     & p(x_{1:t+1} | Z_{t+1})      \nonumber                                                                                                 \\
    % \propto
    %  & p(z_{t+1}|x_{1:t+1},Z_{t})   p(x_{1:t+1},Z_{t})   \nonumber                                                                           \\
    \propto
     & p(z_{t+1}|x_{t+1})   p(x_{1:t+1},Z_{t})   \nonumber                                                                                   \\
    % \propto
    %  & p(z_{t+1}|x_{t+1}) p(x_{t+1}|x_{t})  p(x_{1:t},Z_{t})   \nonumber                                                                     \\
    \propto
     & p(z_{t+1}|x_{t+1}) p(x_{t+1}|x_{t})  p(x_{1:t}|Z_{t}) \nonumber                                                                       \\
    \propto
     & \left[\prod_{k=1}^{t+1} p(z_{k}|x_{k}) \right] \left[\prod_{k=2}^{t+1} p(x_{k}|x_{k-1}) \right] p(x_1) .\label{eq:window_less_than_T}
\end{align}

We sample $\{x^i_{1:t+1}\}_{i=1}^n$ from $p(x_{1:t+1} | Z_{t+1})$ by SVGD. Note that $x^i_{1:t+1} \in \mR^{(t+1)d}$ are the samples from joint distribution and we only take $\{x^i_{t+1} \}_{i=1}^n$ as the output amongst them.

When $t>T$, we can take advantage of the receding window, that is
\begin{align*}
     & p(x_{t+1:t+T} | Z_{t+T})                                             \\
    % \propto
    %  & p(z_{t+T}|x_{t+1:t+T},Z_{t+T-1})   p(x_{t+1:t+T},Z_{t+T-1})          \\
    \propto
     & p(z_{t+T}|x_{t+T})   p(x_{t+1:t+T},Z_{t+T-1})                        \\
    % \propto
    %  & p(z_{t+T}|x_{t+T}) p(x_{t+T}|x_{t+T-1})  p(x_{t+1:t+T-1},Z_{t+T-1})  \\
    \propto
     & p(z_{t+T}|x_{t+T}) p(x_{t+T}|x_{t+T-1})  p(x_{t+1:t+T-1}|Z_{t+T-1}). \\
\end{align*}
% $p(x_{t+1:t+T-1}|Z_{t+T-1})$ hinted the iteration formula. Specifically, we have
It follows that
\begin{align*}
     & p(x_{t+1:t+T} | Z_{t+T})                                                                     \\
    % \propto
    %  & p(z_{t+T}|x_{t+T})   p(x_{t+T}|x_{t+T-1}) p(x_{t+1:t+T-1}|Z_{t+T-1})                         \\
    \propto
     & p(x_{t+1}|Z_{t+1}) \prod _{k=2}^T p(z_{t+k}|x_{t+k})   p(x_{t+k}|x_{t+k-1})                  \\
    % \propto
    %  & p(z_{t+1}|x_{t+1})\int_{x_t} p(x_{t+1} | x_t)p(x_t|Z_t) \prod _{k=2}^T p(z_{t+k}|x_{t+k})   p(x_{t+k}|x_{t+k-1}) \\
    \propto
     & \int_{x_t} p(x_t | Z_t)\prod_{k=1}^T \left(p(z_{t+k}|x_{t+k}) p(x_{t+k} | x_{t+k-1})\right).
\end{align*}
When $p(x_t | Z_t)$ is represented by particles $\{x_t^i\}_{i=1}^n$, the above can be evaluated efficiently and the Stein variational gradient descent \eqref{eq:stein} can be utilized to sample from $p(x_{t+1:t+T} | Z_{t+T})$. With particle-approximated distribution, we have

\begin{align}
     & p(x_{t+1:t+T} | Z_{t+T})  \nonumber                                                                     \\
    \propto
     & \frac{1}{n} \left[\sum_{i=1}^n p(x_t^i | Z_t) p(x_{t+1}|x_{t}^i) \right]   p(z_{t+1}|x_{t+1}) \nonumber \\
     & \times \prod_{k=2}^T p(z_{t+k}|x_{t+k}) p(x_{t+k} | x_{t+k-1}) . \label{eq:window_larger_than_T}
\end{align}

A good initialization can be realized by extending the samples from $p(x_{t:t+T-1} | Z_{t+T-1})$ by using the dynamics \eqref{eq:dyn1}. One potential advantage of this sliding window method is that it reuses some past observations to improve the current estimation and may correct some mistakes made in the past estimations.



\begin{algorithm}[tb]
    \caption{Sliding window Stein particle filtering}
    \label{al:window}
    \begin{algorithmic}
        \IF{$ t = 0$}
        \STATE {\bfseries Input:} initial dist. $p(x_1)$, observation $Z_1$
        % , step size $\epsilon_\ell$
        \STATE { \bfseries Initialize $x^i \sim p(x_1), i=1,2, \ldots, n$}
        \STATE {\bfseries Compute:} $\{\hat{x}^i\}=\text{SVGD}\left(p(x_{1}|Z_{1}),\{x^i \} \right) $ with Algorithm \ref{al:svgd}.
        % \FOR{$\ell=0,\ldots,L-1$}
        % \STATE { $ x_{1,\ell+1}^i=x_{1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{1,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{1}|Z_{1})$ in Equation (\ref{eq:one_step_p1}).
        % }
        % \ENDFOR
        \STATE{\bfseries Output:}$ \{x_{1}^i\}_{i=1}^n=\{\hat{x}^i\}_{i=1}^n$
        % \STATE {\bfseries Output: $\{x_{1}^i\}_{i=1}^n= \{x_{1,L}^i\}_{i=1}^n$}
        %-----------------------------------%
        \ELSIF{$1 \leq t < T$}
        \STATE {\bfseries Input:}
        % $tn$
        particles $\{x_{1:t}^i\}_{i=1}^n \sim p(x_{1:t}|Z_t)$, observations $Z_t$
        % , step size $\epsilon_\ell$
        \STATE { \bfseries Initialize $x^i \sim p(x_{t+1}|x_t^i), i=1,2, \ldots, n$}
        \STATE { \bfseries Concatenate $X^i = \left[x_{1}^i,\ldots x_{t}^i,x^i \right]$}
        \STATE {\bfseries Compute:} $\{\hat{X}^i\}=\text{SVGD}\left(p(x_{1:t+1}|Z_{t+1}),\{X^i \} \right) $.
        % \FOR{$\ell=0,\ldots,L-1$}
        % \STATE { $ x_{1:t+1,\ell+1}^i=x_{1:t+1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{1:t,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{1:t+1}|Z_{t+1})$ in Equation (\ref{eq:window_less_than_T}).
        % }
        % \ENDFOR
        \STATE {\bfseries Output} $\{x_{t+1}^i\}_{i=1}^n$ which are the last dimension particles from $\left\{\widehat{X}^i \right\}$
        and then save $\{x_{1:t+1}^i\}_{i=1}^n=\left\{\widehat{X} \right\}$ for next time input
        %-----------------------------------%
        \ELSIF{$t \geq T$}
        \STATE {\bfseries Input:}
        particles $\{x_{t-T+2:t}^i\}_{i=1}^n \sim p(x_{t-T+2:t}|Z_t)$ , observations $Z_t$
        % , step size $\epsilon_\ell$
        \STATE { \bfseries Initialize $x^i \sim p(x_{t+1}|x_t^i), i=1,2, \ldots, n$}
        % \FOR{$\ell=0,\ldots,L-1$}
        % \STATE { $ x_{t+1,\ell+1}^i=x_{t+1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{t+1,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{t+1}|Z_{t+1})$ in Equation (\ref{eq:stride1_numeric}).
        % }
        % \ENDFOR
        \STATE { \bfseries Concatenate $X^i = \left[x_{t-T+2}^i,\ldots x_{t}^i,x^i \right]$}
        \STATE {\bfseries Compute:} $\{\hat{X}^i\}=\text{SVGD}\left(p(x_{t-T+2:t+1}|Z_{t+1}),\{X^i \} \right) $.
        \STATE {\bfseries Output:} $\{x_{t+1}^i\}_{i=1}^n$ which are the last dimension particles from $\left\{\widehat{X}^i\right\}$
        and then save $\{x_{t-T+3:t+1}^i\}_{i=1}^n=\{\widehat{X}\}$
        % $\{x_{t+1}^i\}_{i=1}^n= \{x_{t+1,L}^i\}_{i=1}^n$
        \ENDIF
    \end{algorithmic}
\end{algorithm}

% \begin{remark}
%     The Sequential Stein particle filtering relies on precise posterior distribution from last timestamp and may suffer from accumulated approximation error.
%     The Sliding window Stein particle filtering however works on a higher dimension space, which may introduce error. So we need to choose them depending on the application scenarios to balance the trade-off.
% \end{remark}

% \begin{remark}
%     % The particles given by our Stein methods have the equal weights. For any $t$, the weight of particle $x_t^i$ is $\frac{1}{n}$. This is different to SIR, which would generate particles with different weights in most time.
%     \jiaojiao{The noise in dynamics Equation \ref{eq:dyn1} is necessary for the Stein particle filtering to work. Otherwise $p(x_{t+1}|x_t^i)$ is a Dirac distribution dominated at}
% \end{remark}

==> Stein filtering/scripts/svgd.tex <==
\subsection{Stein variational gradient descent}
The Stein variational gradient descent (SVGD) \cite{LiuWan16} is a sample-based variational inference technique. It enables efficient sampling from a target probability density $q(x)$ by gradually transforming samples from an arbitrary initial distribution to samples of $q(x)$.

% A reproducing kernel Hilbert space (RKHS) $\cH$ is the closure of $\{h:h(x)=\sum_{j=1}^J r_j k(x,x_j),r_j \in \mR, J\in \mN, x_j \in \mR^d\}$ and $\cH^d$ is the space of vector functions $\mathbf{h}=[h_1,\ldots,h_d]$ with $h_i \in \cH$. Then Kernelized Stein Discrepancy (KSD)  \cite{liu2016kernelized} is
% \begin{align}
%     \mathbb{S}(q,\tilde{q})     & = \| \phi_{q,\tilde{q}}^*\|_{\cH^d }^2,                                                                              \\
%     \phi_{q,\tilde{q}}^*(\cdot) & = \E_{x\sim \tilde{q}} \left[k(x,\cdot) \nabla_x \log \tilde{q}(x)^\tT+ \nabla_x k(x,\cdot)  \right] \label{eq:phi},
% \end{align}
% and have the property
% \begin{align*}
%     \mathbb{S}(q,\tilde{q})=0 \Leftrightarrow  \phi_{q,\tilde{q}}^*=0 \Leftrightarrow \tilde{q}=q
% \end{align*}
% under the assumption that $k(\cdot,\cdot)$ is strictly positive definite \cite{liu2016kernelized,chwialkowski2016kernel}.
% With a simpler distribution $\tilde{q}$, SVGD is aimed at minimizing the KL divergence
% \begin{align*}
%     \tilde{q}^*= \argmin
%     \{\text{KL} (\tilde{q} \| q):=
%     \E_{\tilde{q}} \left[\log \tilde{q}(x)\right]
%     -\E_{\tilde{q}} \left[\log {q}(x)\right]\}.
% \end{align*}
% If we consider $T(x)=x+\epsilon \phi(x)$ and let $T(x) \sim \tilde{q}(x)$ to approximate target $q(x)$, then $T^*(x)=x+\epsilon \phi^*_{q,\tilde{q}}(x)$ is a gradient descent step of the functional
% $\text{KL} (\tilde{q} \| q)$. More explicitly,
% $$\nabla_\epsilon \text{KL} (\tilde{q} \| q) |_{\epsilon=0}=-\mS (\tilde{q},q).$$
Let $\{x^i_\ell\}_{i=1}^n$ be the samples at the $\ell$-th iteration, then the SVGD algorithm evolves the particles with
\begin{equation}\label{eq:stein}
    x^i_{\ell+1} =  x^i_{\ell} + \epsilon_\ell \hat{\phi}^*(x^i_\ell),
\end{equation}
where
% $\hat{\phi }^*(x)$ is the empirical estimation of Equation (\ref{eq:phi}):
\begin{equation}\label{eq:stein_phi}
    \hat{\phi }^*(x)=\frac{1}{n} \sum_{j=1}^n \left[k(x^j_\ell, x)\nabla_{x^j_\ell} \log q(x^j_\ell) + \nabla_{x^j_\ell} k(x^j_\ell, x)\right].
\end{equation}
Here $k(\cdot,\cdot)$ is a positive definite kernel \cite{liu2016kernelized,chwialkowski2016kernel}, e.g., the Gaussian kernel $k(x,x')=\exp(-\frac{1}{h} \|x-x'\|_2^2)$.

\begin{algorithm}[tb]
    \caption{Stein variational gradient descent (SVGD)}
    \label{al:svgd}
    \begin{algorithmic}
        \STATE {\bfseries Input:} A target distribution $q(x)$ and the initialized particles $\{x_{0}^i\}_{i=1}^n$.
        % initial dist. $p(x_1)$, observation $Z_1$, 
        % step size $\epsilon_\ell$, number of iteration $L$.
        % \STATE { \bfseries Initialize $x_{1,0}^i \sim p(x_1), i=1,2, \ldots, n$}
        \FOR{$\ell=0,\ldots,L-1$}
        \STATE { $ x_{\ell+1}^i=x_{\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{\ell}^i)$,
        where $\hat{\phi }^*(x)$ equals to \\
        $\frac{1}{n} \sum_{j=1}^n \left[k(x^j_\ell, x)\nabla_{x^j_\ell} \log q(x^j_\ell) + \nabla_{x^j_\ell} k(x^j_\ell, x)\right].$
        }
        % \STATE { $ x_{1,\ell+1}^i=x_{1,\ell}^i + \epsilon_\ell \hat{\phi}^*(x_{1,\ell}^i)$,
        % where the target distribution $q(x)= p(x_{1}|Z_{1})$ in Equation (\ref{eq:one_step_p1}).
        % }
        \ENDFOR
        \STATE {\bfseries Output:} A set of  particles $\{x_{L}^i\}_{i=1}^n$ that approximates the distribution $q(x)$.
    \end{algorithmic}
\end{algorithm}

Note that the update \eqref{eq:stein_phi} requires only querying $\nabla_x\log q$, thus the normalization constant in $q$ is not important. This property makes it ideal for Bayesian inference problems where the computation of the normalization constant is challenging. We also remark that, unlike the particles in SIR particle filter, which are accompanied by weights, the particles $\{x^i_\ell\}_{i=1}^n$ in SVGD are always equally weighted, thus, no update for weights is needed.

In the mean-field limit, the SVGD \eqref{eq:stein_phi} is the gradient flow of the KL-divergence between the particle distribution and the target distribution $q(x)$ over the velocity field $\hat\phi$ with respect to the norm in a reproducing kernel Hilbert space (RKHS) associated with the kernel $k(\cdot,\cdot)$. Thus, the convergence of SVGD is guaranteed in the mean-field limit. We refer the reader to \cite{LiuWan16} for more detailed discussion on SVGD.
% The RHKS kernel $k(\cdot,\cdot)$ is required to be strictly positive definite to promise the particle distribution converges to the target distribution and 
% We use RBF kernel $k(x,x')=\exp(\frac{1}{h} \|x-x'\|_2^2)$ in this article. We use the pytorch SVGD library \footnote{\url{https://github.com/activatedgeek/svgd}} to implement the algorithm.
